Evidence for mass-dependent peculiar velocities in compact object binaries: Towards better constraints on natal kicks

We compile a catalogue of low-mass and high-mass X-ray binaries, some recently reported binaries that likely host a neutron star (NS) or a black hole (BH), and binary pulsars (a pulsar and a non-degenerated companion) that have measured systemic radial velocities ($\gamma$). Using Gaia and radio proper motions together with $\gamma$, we integrate their Galactic orbits and infer their post-supernova (post-SN) 3D peculiar velocities ($v_\mathrm{pec}^{z=0}$ at Galactic plane crossing); these velocities bear imprint of natal kicks that compact objects received at birth. With the sample totalling 85 objects, we model the overall distribution of $v_\mathrm{pec}^{z=0}$ and find a two-component Maxwellian distribution with a low- ($\sigma_v \approx 21\,\mathrm{km~s^{-1}}$) and a high-velocity ($\sigma_v \approx 107\,\mathrm{km~s^{-1}}$) component. A further comparison between distributions of binary subgroups suggests that binaries hosting high-mass donors/luminous companions mostly have $v_\mathrm{pec}^{z=0}\lesssim 100\,\mathrm{km~s^{-1}}$, while binaries with low-mass companions exhibit a broader distribution that extends up to $\sim 400\,\mathrm{km~s^{-1}}$. We also find significant anti-correlations of $v_\mathrm{pec}^{z=0}$ with binary total mass ($M_\mathrm{tot}$) and orbital period ($P_\mathrm{orb}$), at over 99% confidence. Specifically, our fit suggests $v_\mathrm{pec}^{z=0}\propto M_\mathrm{tot}^{-0.5}$ and $v_\mathrm{pec}^{z=0}\propto P_\mathrm{orb}^{-0.2}$. Discussions are presented on possible interpretation of the correlations in the context of kinematics and possible biases. The sample should enable a range of follow-up studies on compact object binary kinematics and evolution.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
